Generating Automatic Feedback on UI Mockups with Large Language Models

Feedback on user interface (UI) mockups is crucial in design. However, human feedback is not always readily available. We explore the potential of using large language models for automatic feedback. Specifically, we focus on applying GPT-4 to automate heuristic evaluation, which currently entails a human expert assessing a UI's compliance with a set of design guidelines. We implemented a Figma plugin that takes in a UI design and a set of written heuristics, and renders automatically-generated feedback as constructive suggestions. We assessed performance on 51 UIs using three sets of guidelines, compared GPT-4-generated design suggestions with those from human experts, and conducted a study with 12 expert designers to understand fit with existing practice. We found that GPT-4-based feedback is useful for catching subtle errors, improving text, and considering UI semantics, but feedback also decreased in utility over iterations. Participants described several uses for this plugin despite its imperfect suggestions.

==> wordcountanalysis.tex <==
\subsection{Word Count Analysis}
\begin{table}
  \begin{tabular}{|c|p{10cm}|}
    \toprule
    \multicolumn{2}{|c|}{\textbf{ACCURACY}} \tabularnewline \midrule
    \textbf{Accurate Suggestions}& text, clear, label, labels, adding, icon, purpose, function, standard, \textbf{subgroups}, readability, \textbf{visual}, icons, button, spacing, aligned, navigation, \textbf{color}, \textbf{information}, close\\  \midrule
    \textbf{Inaccurate Suggestions} & label, text, clear, labels, adding, icon, button, aligned, icons, \textbf{line}, standard, purpose, close, navigation, readability, \textbf{visible}, spacing, \textbf{rectangles}, function, \textbf{common} \\
    \midrule
    \multicolumn{2}{|c|}{\textbf{HELPFULNESS}} \tabularnewline \midrule
    \textbf{Helpful Suggestions}& clear, text, label, labels, purpose, adding, standard, icon, \textbf{subgroups}, \textbf{visual}, \textbf{color}, function, button, icons, readability, \textbf{graph}, aligned, \textbf{contrast}, close, spacing\\  \midrule
    \textbf{Unhelpful Suggestions} & text, label, clear, button, labels, adding, icon, icons, \textbf{line}, aligned, purpose, standard, function, close, \textbf{input}, \textbf{navigation}, \textbf{visible}, readability, \textbf{relationship}, background \\
  \bottomrule
\end{tabular}
  \caption{Table showing the top 20 common words in accurate, inaccurate, helpful, and unhelpful suggestions. Common words that are in accurate, but not in inaccurate suggestions (and vice versa) are bolded, as well as common words that are in helpful but not in unhelpful suggestions (and vice versa). }
   \label{tab:commonwords}
\end{table}
We carried out a word count analysis to identify characteristics unique to suggestions that are rated as accurate, inaccurate, helpful, and unhelpful. ``Accurate" and ``inaccurate" refer to suggestions given that rating on the accuracy scale (``accurate", ``partially", ``inaccurate"). ``Helpful" refers to a rating of at least 4 on the helpfulness Likert scale (5 is considered ``very helpful") and ``unhelpful" refers to ratings of 1. We then computed the top 20 most frequently occurring words for each category, filtering out stop words and other uninformative words like ``interface” and ``guideline”. We then look at common words that are in accurate suggestions but not in inaccurate suggestions, and vice versa, and also do this for helpful and unhelpful suggestions. Table \ref{tab:commonwords} contains the top 20 words in each category, with the identified unique words bolded. We carried out this analysis on the LLM suggestions from the Usage Study, as there is a higher portion of lower-rated suggestions due to the LLM’s worse performance in later rounds.

The results of this word analysis support our quantitative and qualitative findings. The words that are common in accurate suggestions, but uncommon in inaccurate suggestions include \textit{subgroups}, \textit{visual}, \textit{color}, and \textit{information}. \textit{subgroups} could be due to the fact that the hierarchical subgrouping guideline had high accuracy ratings in the usage study (Figure \ref{fig:guidelineperformancevalidation}. Words that are common in inaccurate suggestions, but uncommon in accurate suggestions are \textit{line}, \textit{visible}, \textit{rectangles}, and \textit{common}. \textit{rectangles} probably appears because poorly named elements (pictures, button bounding boxes, etc) in the layers panel were called “Rectangle N”, where "N" is some number, and the LLM may have had a difficult time reasoning with poorly named elements. Furthermore \textit{common} and \textit{line} could be due to the times when the LLM incorrectly called out elements that are center aligned to not be "aligned along a common line" due to different bounding box sizes. 

Words that are common in helpful suggestions but uncommon in unhelpful suggestions include \textit{subgroups}, \textit{visual}, \textit{color}, \textit{graph}, \textit{contrast}, and \textit{spacing}. The Hierarchical Subgrouping guideline also had high helpfulness ratings, which could explain \textit{subgroups}. Participants also stated that the LLM was useful for catching \textit{visual} details like \textit{color} \textit{contrast} and \textit{spacing}. Finally, words that are common in unhelpful suggestions but are uncommon in helpful suggestions include \textit{line}, \textit{input}, \textit{navigation}, \textit{understand}, \textit{visible}, and \textit{relationship}. Participants often found suggestions to add labels to icons in the bottom \textit{navigation} bar unhelpful as those icons were usually quite common. 

While there is overlap amongst the top 20 common words in the suggestions from different rating categories, some words are used in various types of heuristics that cover a wide range of issues. For instance ``text" is in the Top 20 words for every category, as shown in Table \ref{tab:commonwords} and can touch on issues like grammatical errors, missing text labels, or unclear text labels, which have a variety of correctness. 
